Grounding Everything: Emerging Localization Properties in Vision-Language Transformers

Vision-language foundation models have shown remarkable performance in various zero-shot settings such as image retrieval, classification, or captioning. But so far, those models seem to fall behind when it comes to zero-shot localization of referential expressions and objects in images. As a result, they need to be fine-tuned for this task. In this paper, we show that pretrained vision-language (VL) models allow for zero-shot open-vocabulary object localization without any fine-tuning. To leverage those capabilities, we propose a Grounding Everything Module (GEM) that generalizes the idea of value-value attention introduced by CLIPSurgery to a self-self attention path. We show that the concept of self-self attention corresponds to clustering, thus enforcing groups of tokens arising from the same object to be similar while preserving the alignment with the language space. To further guide the group formation, we propose a set of regularizations that allows the model to finally generalize across datasets and backbones. We evaluate the proposed GEM framework on various benchmark tasks and datasets for semantic segmentation. It shows that GEM not only outperforms other training-free open-vocabulary localization methods, but also achieves state-of-the-art results on the recently proposed OpenImagesV7 large-scale segmentation benchmark.

==> tabs/self_self_kmeans.tex <==

\begin{figure*}[t]
    \centering
    \begin{minipage}{\textwidth}
    \begin{minipage}[t]{0.3\textwidth}
    \vspace{-7em}

    
    \resizebox{1\columnwidth}{!}{
\begin{tabular}{c c c c c}
\toprule 
Projection & Norm.+Temp.  & VOC & Context \\ 
\midrule 
CLIP    & - & 10.4 & 7.7 \\
\midrule 
v-v  & \color{lightgray}\ding{55}  & 41.9 & 30.5 \\
k-k & \color{lightgray}\ding{55}  &43.9& 31.0\\
q-q & \color{lightgray}\ding{55}  & 43.8& 30.8\\
\hline
qkv & \color{lightgray}\ding{55} & 43.1& 30.7\\
\midrule
v-v &\ding{51} & 44.4 & 31.9 \\
k-k &\ding{51} & 44.8& 32.0\\
q-q &\ding{51} &44.7 & 31.5\\
\hline
qkv &\ding{51} & 45.1 & 32.3 \\
\bottomrule
\end{tabular}
}
\captionof{table}{mIoU for v-v, k-k, and q-q attention and qkv ensemble on PascalVOC and PascalContext with and without L$^2$-Norm and adaptive temperature.

}
\label{tab:attn_types}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\textwidth}
    \vspace{-7em}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{c c c c}
    \toprule 
    Method  & iter & VOC & Context \\ 
    \midrule
    CLIP        & - & 10.4 & 7.7 \\
    \hline
       CS &  0 & 41.2 & 30.5\\
      GEM & 0 & 45.1 &31.5 \\
      GEM & 1 & \underline{45.5} & \textbf{32.6}\\
      GEM & 2 &  \textbf{46.2}& \underline{31.9}\\
      GEM & 3 & 45.6 & 31.1\\
    \bottomrule
    \end{tabular}
    }
    \captionof{table}{Influence of the number of iterations for the self-self-attention in the GEM architecture.} \label{tab:kmeans}
    \end{minipage}
    \hfill
    \begin{minipage}{0.35\textwidth}
    \centering

    \includegraphics[width=\linewidth]{images/softmax_clustering_viz_no_kmeans.pdf}
    \captionof{figure}{Comparison of self-self attention for different numbers of iterations and temperature on 20 vectors.
    \vitto{unclear figure, you have to tell what a cell of one of these matrices represents (I assume some form of similarity between two $x$ tokens, but you have to tell it explicitly.}
    }
    \label{fig:softmax-clustering}% 
    \end{minipage}
    \end{minipage}
\end{figure*}


